Not All Poisons are Created Equal: Robust Training against Data Poisoning

Data poisoning causes misclassification of test time target examples by injecting maliciously crafted samples in the training data. Existing defenses are often effective only against a specific type of targeted attack, significantly degrade the generalization performance, or are prohibitive for standard deep learning pipelines. In this work, we propose an efficient defense mechanism that significantly reduces the success rate of various data poisoning attacks, and provides theoretical guarantees for the performance of the model. Targeted attacks work by adding bounded perturbations to a randomly selected subset of training data to match the targets' gradient or representation. We show that: (i) under bounded perturbations, only a number of poisons can be optimized to have a gradient that is close enough to that of the target and make the attack successful; (ii) such effective poisons move away from their original class and get isolated in the gradient space; (iii) dropping examples in low-density gradient regions during training can successfully eliminate the effective poisons, and guarantees similar training dynamics to that of training on full data. Our extensive experiments show that our method significantly decreases the success rate of state-of-the-art targeted attacks, including Gradient Matching and Bullseye Polytope, and easily scales to large datasets.

==> problem.tex <==
\section{Training with Poisoned Data}
Let $\mathcal{D}_c=\{(x_c^{(j)},y_c^{(j)})\}_{j=1}^n$ be the set of all clean training data, and let $\mathcal{D}_p = \{(x^{(j)}_p,y_p^{(j)})\}^{m}_{j=1}$ denote the set of $m$ poison examples with their corresponding labels. Poison labels $y_p^{(j)}$ may be clean, i.e., they still appear natural and properly labeled upon human inspection.
% , or they may be corrupted, i.e., flipped to another label. We denote by %$V=\{1,\cdots,n, n+1,\cdots n+j \}$ 
$V_c, V_p$ index sets of the clean and poisoned data, respectively. $V=\{V_c \cup V_p\}$ is the index set of the entire training data, containing the poisoned examples. 
% Following the benchmark setting defined in \cite{schwarzschild2020just}, we focus on targeted attacks whose goal is to make one target test example $x_t$ to be misclassified as a specified class. 
\ba{discuss attack example, defense assumptions, etc}

% with corresponding clean base image $\{x_b^{(j)}\}^J_{j=1}$. Let $x_t$ be the target image. Labels are denoted by $y$ and $Y$ for a single image and a set of images, respectively, and are indexed to match the data. 

%
% We consider training both linear models and neural networks. For neural networks, we consider end-to-end training scenarios, when all layers are trainable, as well as transfer learning from a pre-trained network, in which a pre-trained feature extraction network is used, and only the final network (softmax) layer is trained to adapt the network to a new task.

%. where the pre-training data and fine-tuning data are not from the same datasets and do not contain the same classes

%Suppose that the model is trained by minimizing the squared loss over the noisy training dataset $\mathcal{D}=\{(\x_i, y_i)\}_{i=1}^n$:
%\begin{equation}
%    \mathcal{L}(\W)=\frac{1}{2}\sum_{i\in V} (y_i - f(\W, \x_i))^2,
%\end{equation}
%
%where $V\!\!=\!\!\{1,\cdots,n\}$ is the set of training examples.
% Supposed $f$ is a model with parameters $W$, and that the network is trained by minimizing the loss $\mathcal{L}(W,X)= \sum_{i\in V}\mathcal{L}_i(W)$ over the entire set of clean and poisoned training examples, and $\mathcal{L}_i(W)=l((x_i,y_i), W)$ is the loss associated with example $i\in V$.
% %$\mathcal{D}=\mathcal{D}_c\cup \mathcal{D}_p$.
% %We apply gradient descent with a constant learning rate $\eta$, starting from an initial point $\W_0$ to minimize $\mathcal{L}(\W)$. 
% The gradient descent iterations take the form
% %
% \begin{equation}\label{eq:GD}
% \begin{split}
%     W_{\tau+1}&=W_{\tau}-\eta \nabla \mathcal{L}(W_\tau,X). %\\ 
%     %& \nabla \mathcal{L}(\W,\X)=\Jc^T(\W,\X)(f(\W,\X)-\y),
% \end{split}
% \end{equation}
%
%where $\Jc(\W,\X)\in \R^{n\times m}$ is the Jacobian matrix associated with the nonlinear mapping $f$ defined as
%\begin{equation}
%    \mathcal{J}(\W,\X)=\big[ \frac{\partial f(\W, \x_1)}{\partial \W} ~~\cdots~~ \frac{\partial f(\W, \x_n)}{\partial \W} \big]^T,
%\end{equation}
% \subsection{Targeted Attacks}
% We consider two types of indiscriminate attacks, label flipping and maximum loss, for training linear models and two types of clean-label targeted attacks, feature collision and hidden trigger backdoor, for training neural networks:

% \paragraph{Label Flipping (LF)}
% Poisons are a set of random data points for which the label is randomly flipped to another class.

% \paragraph{Maximum Loss (ML)}
% In iteration $j$, it alternates between finding the worst attack point in the feasible set $\mathcal{F}$ that maximizes the training loss
% \begin{equation}
% (x_p^{(j)}, y_p^{(j)})={\arg\max}_{(x,y)\in \mathcal{F}}\allowbreak l((x,y), W_j),
% \end{equation}
% with respect to the current model $\W_j$, and updating the model in the direction of the attack point. 
%, normalized by a parameter $\mu$. %, producing
% \begin{equation}
% \W_{\tau+1}=[\W_\tau-\nabla \mathcal{L}(\W_\tau)-\epsilon \nabla l((\x_i,y_i), \W_\tau)]/\mu.
% \end{equation}
%where $\mu$ is a normalization factor.


%
